Ruby: State-of-the-Art Potency Prediction across Discovery Regimes Using Learned Structural Representations

Small-molecule drug discovery proceeds through repeated design-make-test-analyze cycles. The goal is often to maximize potency while keeping other properties within the ranges required for a viable therapeutic candidate. Compound prioritization places different demands on computational methods as drug discovery progresses from hit identification through hit-to-lead and lead optimization, with changing computational budgets and increasing amounts of on-target experimental data. We introduce Ruby, a Robust Universal Binding affinitY predictor that uses intermediate representations from the structural foundation model Pearl without requiring an explicit binding pose for every compound. Ruby is trained on proprietary data plus GenesisPotency-2026, an audited public-source potency training dataset released for academic and commercial use under a CC BY-SA 4.0 license with row-level provenance and audit annotations. Ruby achieves the highest aggregate early enrichment across seven public hit-identification targets among evaluated methods, with adjustable inference effort trading off enrichment and computational cost over more than two orders of magnitude. Ruby achieves the highest average correlations across four public benchmarks: OpenFE, CASP16, FEP+ 4, and OpenBind. Ruby significantly outperforms other methods in zero-shot prediction across eight biochemical and cellular assays from five ongoing Genesis-Incyte programs, widening its performance advantage relative to the public benchmarks. Ruby continues to improve more than other methods when all are given the opportunity to recalibrate using earlier assay measurements. Together, these contributions provide an annotated training resource for the field and a state-of-the-art potency predictor for broad screening, prioritization within related chemical series, and assay-specific prediction as experimental measurements accumulate.

==> generated/status.tex <==
\ppsetstatus{cost}{}
\ppsetstatus{hitid}{}
\ppsetstatus{incyte_detail}{}
\ppsetstatus{programs}{}
\ppsetstatus{scaling}{}
\ppsetstatus{series}{}

